Exploring Diffusion Time-steps for Unsupervised Representation Learning

Representation learning is all about discovering the hidden modular attributes that generate the data faithfully. We explore the potential of Denoising Diffusion Probabilistic Model (DM) in unsupervised learning of the modular attributes. We build a theoretical framework that connects the diffusion time-steps and the hidden attributes, which serves as an effective inductive bias for unsupervised learning. Specifically, the forward diffusion process incrementally adds Gaussian noise to samples at each time-step, which essentially collapses different samples into similar ones by losing attributes, e.g., fine-grained attributes such as texture are lost with less noise added (i.e., early time-steps), while coarse-grained ones such as shape are lost by adding more noise (i.e., late time-steps). To disentangle the modular attributes, at each time-step t, we learn a t-specific feature to compensate for the newly lost attribute, and the set of all 1,...,t-specific features, corresponding to the cumulative set of lost attributes, are trained to make up for the reconstruction error of a pre-trained DM at time-step t. On CelebA, FFHQ, and Bedroom datasets, the learned feature significantly improves attribute classification and enables faithful counterfactual generation, e.g., interpolating only one specified attribute between two images, validating the disentanglement quality. Codes are in https://github.com/yue-zhongqi/diti.

==> figures/fig_bed-fulldim.tex <==
\begin{figure}[!tbp]
  \centering
  \includegraphics[width=1.0\linewidth]{figures/bed-fulldim.pdf}
  \caption{Comparsions of PDAE (top row) and DiTi (bottom row)'s interpolation results on Bedroom using all dimensions of the feature $\mathbf{z}$.}
  \label{suppfig:bed-fulldim}
\end{figure}

==> figures/fig_bed-interp.tex <==
\begin{figure}[!tbp]
  \centering
  \includegraphics[width=1.0\linewidth]{figures/bed-interp.pdf}
  \caption{Comparisions on PDAE (top row) and DiTi (bottom row)'s counterfactual generation results on Bedroom using 3 feature subsets. For each image pair in each subset, the original images, $\mathbf{x}_0^1, \mathbf{x}_0^2$ are placed in the top left corner and bottom right corner, and interpolated towards its counterpart in four scales (1/4, 2/4, 3/4 and 1) respectively.}
  \label{suppfig:bed-interp}
\end{figure}

==> figures/fig_bed-manip.tex <==
\begin{figure}[!tbp]
  \centering
  \includegraphics[width=0.8\linewidth]{figures/bed-manip.pdf}
  \caption{Comparsions of PDAE (left column) and DiTi (right column)'s modular manipulation results on Bedroom. For both methods, we use ProbMask to constrain the classifier weight such that it has $d'=32$ non-zero dimensions.}
  \label{suppfig:bed-manip}
\end{figure}

==> figures/fig_celeba-fulldim.tex <==
\begin{figure}[!tbp]
  \centering
  \includegraphics[width=.5\linewidth]{figures/celeba-fulldim.pdf}
  \caption{Comparsions of PDAE (top row) and DiTi (bottom row)'s manipulation results on CelebA using all dimensions of the feature $\mathbf{z}$.}
  \label{suppfig:celeba-fulldim}
\end{figure}

==> figures/fig_celeba-manip.tex <==
\begin{figure}[!tbp]
  \centering
  \includegraphics[width=0.8\linewidth]{figures/celeba-manip.pdf}
  \caption{Comparsions of PDAE and DiTi's modular manipulation results on CelebA. The center image in each group of 5 images corresponds to the original image $\mathbf{x}_0$. We use $d'=128$ as the dimension of ProbMask on ``Wearing Hat'' attribute and $d'=16$ for the rest.}
  \label{suppfig:celeba-manip}
\end{figure}

==> figures/fig_ffhq-fulldim.tex <==
\begin{figure}[!tbp]
  \centering
  \includegraphics[width=1.0\linewidth]{figures/ffhq-fulldim.pdf}
  \caption{Comparsions of PDAE (top row) and DiTi(bottom row)'s interpolation results on FFHQ using all dimensions of the feature $\mathbf{z}$.}
  \label{suppfig:ffhq-fulldim}
\end{figure}

==> figures/fig_ffhq-interp.tex <==
\begin{figure}[!tbp]
  \centering
  \includegraphics[width=1.0\linewidth]{figures/ffhq-interp.pdf}
  \caption{DiTi's counterfactual generation results on FFHQ. For every image pair, the original images are placed on the top left and bottom right corners, and interpolated on a specific subset of $\{\mathbf{z}_i\}_{i=1}^k$ to gradually transition towards its counterpart with four scales (1/4, 2/4, 3/4 and 1). Each row is the result of interpolating on a subset, with the subset range displayed on the left.}
  \label{suppfig:ffhq-interp}
\end{figure}

==> tables/std.tex <==
\begin{table}[h!]
      \centering
            \setlength\extrarowheight{1pt}
            \scalebox{0.9}
            {\begin{tabular}{clccc}
                \toprule
                &Methods & \textbf{AP}\ $\uparrow$ & \textbf{Pearson's r}\ $\uparrow$ & \textbf{MSE}\ $\downarrow$ \\
                \midrule
                \multicolumn{1}{c}{\multirow{5}{*}{\rotatebox{90}{\textbf{CelebA}}}}
                &PDAE~\cite{zhang2022unsupervised} & 60.2 $\pm$ 0.013  & 0.596 $\pm$ 5.9e-4  & 0.410 $\pm$ 6.8e-4    \\
                &SimCLR~\cite{chen2020simple} & 59.7 $\pm$ 0.015 & 0.474 $\pm$ 3.7e-3 & 0.603 $\pm$ 3.1e-3    \\
                &SimCLR$-$Aug~\cite{chen2020simple} & 34.7 $\pm$ 0.063 & 0.176 $\pm$ 3.3e-3 & 0.717 $\pm$ 2.2e-3    \\
                &SimSiam~\cite{chen2020exploring} & 51.7 $\pm$ 0.152 & 0.464 $\pm$ 7.2e-3 &    0.525 $\pm$ 4.5e-3  \\
                &\textbf{DiTi (Ours)} & 62.3 $\pm$ 0.083 & 0.617 $\pm$ 4.6e-4 & 0.392 $\pm$ 1.0e-3     \\
                \midrule
                \multicolumn{1}{c}{\multirow{3}{*}{\rotatebox{90}{\textbf{FFHQ}}}}
                &PDAE~\cite{zhang2022unsupervised} & 59.7 $\pm$ 0.030 & 0.603 $\pm$ 7.1e-4 & 0.416 $\pm$ 1.2e-3     \\
                &SimCLR~\cite{chen2020simple} & 60.8 $\pm$ 0.025 & 0.481 $\pm$ 4.5e-3 & 0.638 $\pm$ 1.9e-2   \\
                &\textbf{DiTi (Ours)} & 61.4 $\pm$ 0.029 & 0.622 $\pm$ 3.9e-4 & 0.384 $\pm$ 2.9e-4   \\
                \bottomrule
            \end{tabular}}
        \vspace{+2mm}
        %\captionsetup{width=0.94\linewidth}
        \captionof{table}{AP (\%) on CelebA attribute classification and Pearson's r, MSE on LFW attribute regression. Supplementary to Table 1. Standard deviations are computed on 5 independent runs.}
         \label{tab:std}
         \vspace{-4mm}
\end{table}
